DreamDissector: Learning Disentangled Text-to-3D Generation from 2D Diffusion Priors

Text-to-3D generation has recently seen significant progress. To enhance its practicality in real-world applications, it is crucial to generate multiple independent objects with interactions, similar to layer-compositing in 2D image editing. However, existing text-to-3D methods struggle with this task, as they are designed to generate either non-independent objects or independent objects lacking spatially plausible interactions. Addressing this, we propose DreamDissector, a text-to-3D method capable of generating multiple independent objects with interactions. DreamDissector accepts a multi-object text-to-3D NeRF as input and produces independent textured meshes. To achieve this, we introduce the Neural Category Field (NeCF) for disentangling the input NeRF. Additionally, we present the Category Score Distillation Sampling (CSDS), facilitated by a Deep Concept Mining (DCM) module, to tackle the concept gap issue in diffusion models. By leveraging NeCF and CSDS, we can effectively derive sub-NeRFs from the original scene. Further refinement enhances geometry and texture. Our experimental results validate the effectiveness of DreamDissector, providing users with novel means to control 3D synthesis at the object level and potentially opening avenues for various creative applications in the future.

==> figures_tex/concept_discrepancy.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/concept_discrepancy.pdf}
    \caption{
        \textbf{Concept discrepancy in diffusion models.} 
        The text prompt is \textit{``A chimpanzee looking through a telescope"}. The ambiguity of the disentanglement arises because the tripod-mounted telescope is situated in the dominant feature space of the T2I diffusion model for the prompt \textit{``a telescope"}, whereas the handheld telescope occupies a marginal feature space.
    }
    % \vspace{-2mm}
    \label{fig:discrepancy}
\end{figure}

==> figures_tex/deep_concept_mining.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/dcm_yswu.pdf}\\
    % \vspace{-2mm}
    \caption{
        \textbf{Overview of Deep Concept Mining~(DCM)}. We finetune the text embedding and the T2I diffusion model with the masked diffusion loss~(Eq.~\ref{eq:masked_diffusion}).
    }
    % \vspace{-2mm}
    \label{fig:deep_concept_mining}
\end{figure}

==> figures_tex/result.tex <==
\begin{figure*}[th!]
    \centering
    \includegraphics[width=\linewidth]{example-image-a} \\
    \vspace{-2mm}
    \caption{Illustration of using different strategies for disentangling the NeRF.
    }
    \label{fig:result}
\end{figure*}

==> figures_tex/teaser.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/teaser_new.png}\\
    % \vspace{-2mm}
    \caption{
    \textbf{Results and applications of our DreamDissector.} \textbf{Top left}: DreamDissector can generate multiple independent textured meshes with plausible interactions. \textbf{Top right}: DreamDissector facilitates text-guided texturing at the object level. \textbf{Bottom left}: DreamDissector enhances convenient manual user geometry editing through simple operations, such as dragging and duplicating. \textbf{Bottom right}: DreamDissector facilitates text-guided controllable object replacement.
    }
    \label{fig:teaser}
\end{figure}
